A finite time analysis of distributed Q-learning

Multi-agent reinforcement learning (MARL) has witnessed a remarkable surge in interest, fueled by the empirical success achieved in applications of single-agent reinforcement learning (RL). In this study, we consider a distributed Q-learning scenario, wherein a number of agents cooperatively solve a sequential decision making problem without access to the central reward function which is an average of the local rewards. In particular, we study finite-time analysis of a distributed Q-learning algorithm, and provide a new sample complexity result of $\tilde{\mathcal{O}}\left( \min\left\{\frac{1}{\epsilon^2}\frac{t_{\text{mix}}}{(1-\gamma)^6 d_{\min}^4 } ,\frac{1}{\epsilon}\frac{\sqrt{|\gS||\gA|}}{(1-\sigma_2(\boldsymbol{W}))(1-\gamma)^4 d_{\min}^3} \right\}\right)$ under tabular lookup

==> prelim/distributed.tex <==

% Several useful properties regarding $\mTheta$ and $\bar{\mW}$ are in order:
% \begin{align*}
%     \bar{\mW}\mTheta =& \bar{\mW}- \frac{1}{N}(\bm{1}_N\bm{1}_N^{\top})\otimes\mI_{|\gS||\gA|}= \left( \mW-\frac{1}{N}\bm{1}_N\bm{1}_N^{\top} \right) \otimes \mI_{|\gS||\gA|},\\
%     \mTheta^2 =& \mI_{N||\gS||\gA|}-\frac{1}{N}(\bm{1}_N\bm{1}_N^{\top})\otimes\mI_{|\gS||\gA|},
% \end{align*}
% and noting that $\bar{\mW}\mTheta$ is a symmetric matrix, we have $\bar{\mW}\mTheta=\mTheta\bar{\mW}$.

